Characterizing Observed Extra Mixing Trends in Red Giants using the Reduced Density Ratio from Thermohaline Models

Observations show an almost ubiquitous presence of extra mixing in low-mass upper giant branch stars. The most commonly invoked explanation for this is thermohaline mixing. One-dimensional stellar evolution models include various prescriptions for thermohaline mixing, but the use of observational data directly to discriminate between thermohaline prescriptions has thus far been limited. Here, we propose a new framework to facilitate direct comparison: Using carbon-to-nitrogen measurements from the SDSS-IV APOGEE survey as a probe of mixing and a fluid parameter known as the reduced density ratio from one-dimensional stellar evolution programs, we compare the observed amount of extra mixing on the upper giant branch to predicted trends from three-dimensional fluid dynamics simulations. Using this method, we are able to empirically constrain how mixing efficiency should vary with the reduced density ratio. We find the observed amount of extra mixing is strongly correlated with the reduced density ratio and that trends between reduced density ratio and fundamental stellar parameters are robust across choices for modeling prescription. We show that stars with available mixing data tend to have relatively low density ratios, which should inform the regimes selected for future simulation efforts. Finally, we show that there is increased mixing at low reduced density ratios, which is consistent with current hydrodynamical models of thermohaline mixing. The introduction of this framework sets a new standard for theoretical modeling efforts, as validation for not only the amount of extra mixing, but trends between the degree of extra mixing and fundamental stellar parameters is now possible.

==> mesa_models/HB_calculation_Brown_Garaud_Stellmach_13_coeff1.0e+00_alpha1.6000_Z0.01051793_M1.1/inlist_pgstar_thermohaline <==
&pgstar

pgstar_show_age_in_years = .false.
pgstar_show_age_in_seconds = .true.

! Kippenhahn diagram history plot

Kipp_win_flag = .true.

! window properties
Kipp_win_width = 9
Kipp_win_aspect_ratio = 0.74
Kipp_title = 'Kippenhahn'

! y axis limits
Kipp_mass_max = 0.4
Kipp_mass_min = 0.22
Kipp_show_mass_boundaries = .true.
Kipp_xaxis_name='model_number'

! x axis limits
!Kipp_xmax = -1              ! maximum step number.  negative means use default.
!Kipp_xmin = -1            ! minimum step number.  negative means use default.
!Kipp_max_width = -1         ! only used if > 0.  causes xmin to move with xmax.

! file output
Kipp_file_flag = .false.
Kipp_file_dir = 'Kipp'
Kipp_file_prefix = 'kipp_'
!Kipp_file_cnt = 1          ! output when mod(model_number,Kipp_file_cnt)==0
Kipp_file_width = -1        ! (inches) negative means use same value as for window
Kipp_file_aspect_ratio = -1 ! negative means use same value as for window
file_device = 'png'         ! options 'png' and 'vcps' for png and postscript
file_extension = 'png'      ! common names are 'png' and 'ps'


!--------------------------------------------------------------------------------------


! Abundance profile plot

Abundance_win_flag = .true.


! isotopes to plot
Abundance_num_isos_to_show = 2
Abundance_which_isos_to_show(1) = 'h1'
Abundance_which_isos_to_show(2) = 'he3'


! window properties
Abundance_win_width =
Abundance_win_aspect_ratio =

Abundance_xleft =
Abundance_xright =
Abundance_ybot =
Abundance_ytop =
Abundance_txt_scale =
Abundance_title =

! isotopes to plot
Abundance_num_isos_to_show = 8
Abundance_which_isos_to_show(1) = 'h1'
Abundance_which_isos_to_show(2) = 'he3'
Abundance_which_isos_to_show(3) = 'c12'
Abundance_which_isos_to_show(4) = 'o16'
Abundance_which_isos_to_show(5) = 'n14'
Abundance_which_isos_to_show(6) = 'c13'
Abundance_which_isos_to_show(7) = 'he4'
Abundance_which_isos_to_show(8) = 'Li7'

! number and size of isotope labels along curves
num_abundance_line_labels =
Abundance_line_txt_scale_factor =

! number and size of isotopes on legend
Abundance_legend_max_cnt = 0
Abundance_legend_txt_scale_factor =

! xaxis name and orientation
Abundance_xaxis_name =
Abundance_xaxis_reversed =

! xaxis limits
Abundance_xmin = 0.2
Abundance_xmax = 0.4

! yaxis limits
Abundance_log_mass_frac_min = -3
Abundance_log_mass_frac_max = 0.1

!------------------------------------------------------------------------------------

! Profile Panel





Profile_Panels1_num_panels = 3
Profile_Panels1_txt_scale = 1.0
Profile_Panels1_title = 'Diagnostic'
Profile_Panels1_win_flag = .true.
Profile_Panels1_xaxis_name = 'logtau' !'logT'
Profile_Panels1_xmin = -0.6 !4 ! only used if /= -101d0
Profile_Panels1_xmax = 10   ! only used if /= -101d0
Profile_Panels1_yaxis_name(:) = 'opacity'
Profile_Panels1_ymin(:) = -101! only used if /= -101d0
Profile_Panels1_ymax(:) = -101 ! only used if /= -101d0
Profile_Panels1_other_yaxis_name(:) = 'logRho'
Profile_Panels1_other_ymin(:) = -101 ! only used if /= -101d0
Profile_Panels1_other_ymax(:) = -101 ! only used if /= -101d0
Profile_Panels1_show_grid = .true.
Profile_Panels1_xaxis_reversed = .false.

Profile_Panels1_yaxis_name(2) = 'entropy' !'entropy'
Profile_Panels1_other_yaxis_name(2) = 'extra_heat' !mass'
Profile_Panels1_ymin(2) = !14! only used if /= -101d0
Profile_Panels1_ymax(2) = !19 ! only used if /= -101d0
Profile_Panels1_other_ymin(2) = !14
Profile_Panels1_other_ymax(2) = !19
Profile_Panels1_yaxis_name(3) = 'logT' ! pgas_div_ptotal' ! 'logtau'
Profile_Panels1_other_yaxis_name(3) = 'log_L_div_Ledd' !'log_L_div_Ledd'


! ----------------------

pgstar_lw = 6 ! integer

! ----------------------


! Mixing profile

Mixing_win_flag = .true.

! window properties
Mixing_win_width =
Mixing_win_aspect_ratio =
Mixing_title = 'Mixing'

! x-axis
Mixing_xaxis_name = 'mass'
Mixing_xaxis_reversed = .false.
Mixing_xmin =  0.24
Mixing_xmax =  0.5

! y-axis
Mixing_ymin = 0
Mixing_ymax = 18
Mixing_dymin =

! file output
Mixing_file_flag = .false.
Mixing_file_dir = 'Mixing'
Mixing_file_prefix = 'mixing_'
!Mixing_file_cnt = 5           ! output when mod(model_number,Mixing_file_cnt)==0
Mixing_file_width = -1        ! (inches) negative means use same value as for window
Mixing_file_aspect_ratio = -1 ! negative means use same value as for window
file_device = 'png'         ! options 'png' and 'vcps' for png and postscript respectively
file_extension = 'png'      ! common names are 'png' and 'ps'

! ---------------------

  !### Profile_Panels4

         Profile_Panels4_win_flag = .true.
         Profile_Panels4_win_width = 6
         Profile_Panels4_show_grid = .false.

         ! setup default plot
         Profile_Panels4_win_aspect_ratio = 0.75
         !Profile_Panels4_txt_scale = 0.9
         Profile_Panels4_ybot = 0.1
         Profile_Panels4_ytop = 0.9
         Profile_Panels4_title = 'Dynamo'

         Profile_Panels4_xaxis_name = 'radius_cm'
         Profile_Panels4_xmin = 2.5d8 ! only used if /= -101d0
         Profile_Panels4_xmax = 3.85d8 ! only used if /= -101d0



         Profile_Panels4_num_panels = 1
         Profile_Panels4_yaxis_name(1) = 'Dynamo'
         !Profile_Panels4_yaxis_name(2) = 'Power'
         !Profile_Panels4_yaxis_name(3) = 'Mixing'
         !Profile_Panels4_yaxis_name(4) = 'Dynamo'

         ! file output
         Profile_Panels4_file_flag = .false.
         Profile_Panels4_file_dir = 'png'
         Profile_Panels4_file_prefix = 'profile_Panels4_'
        ! Profile_Panels4_file_cnt = 5 ! output when mod(model_number,Profile_Panels4_file_cnt)==0
         Profile_Panels4_file_width = -1 ! (inches) negative means use same value as for window
         Profile_Panels4_file_aspect_ratio = -1 ! negative means use same value as for window


!------------ Text_Summary windows

Text_Summary1_win_flag = .true.
Text_Summary1_win_width = 5
Text_Summary1_win_aspect_ratio = 0.13

Text_Summary1_xleft = 0.06
Text_Summary1_xright = 1.02
Text_Summary1_ybot = 0.0
Text_Summary1_ytop = 1.0
Text_Summary1_txt_scale = 4.0
Text_Summary1_title = ''

Text_Summary1_num_rows = 3 ! <= 20
Text_Summary1_num_cols = 4 ! <= 20
Text_Summary1_name(:,:) = ''

Text_Summary1_name(1,1) = 'time_step'
Text_Summary1_name(1,2) = 'num_zones'
Text_Summary1_name(1,3) = 'star_mass'
Text_Summary1_name(1,4) = 'star_mdot'

Text_Summary1_name(2,1) = 'log_total_angular_momentum'
Text_Summary1_name(2,2) = 'center_omega'
Text_Summary1_name(2,3) = 'surf_avg_omega'
Text_Summary1_name(2,4) = 'surf_avg_v_rot'

Text_Summary1_name(3,1) = 'log_Teff'
Text_Summary1_name(3,2) = 'photosphere_L'
Text_Summary1_name(3,3) = 'photosphere_r'
Text_Summary1_name(3,4) = 'star_age'


!------------------------------------------------------------------------------------


Kipp_win_flag = .false.
Abundance_win_flag = .false.
Profile_Panels1_win_flag = .false.
Profile_Panels4_win_flag = .false.
Mixing_win_flag = .false.
Dynamo_win_flag = .false.
Text_Summary1_win_flag = .false.

!------------------------------------------------------------------------------------

Grid1_win_flag = .true.
Grid1_win_width = 12
Grid1_win_aspect_ratio = 0.65

Grid1_num_cols = 3 ! divide plotting region into this many equal width cols
Grid1_num_rows = 2 ! divide plotting region into this many equal height rows
Grid1_num_plots = 6 ! <= 10

Grid1_xleft = 0.07 ! fraction of full window width for margin on left
Grid1_xright = 0.98 ! fraction of full window width for margin on right
Grid1_ybot = 0.05 ! fraction of full window width for margin on bottom
Grid1_ytop = 0.92 ! fraction of full window width for margin on top


Grid1_plot_name(1) = 'Text_Summary1'
Grid1_plot_row(1) = 1           ! number from 1 at top
Grid1_plot_rowspan(1) =1       ! plot spans this number of rows
Grid1_plot_col(1) =  1          ! number from 1 at left
Grid1_plot_colspan(1) = 3       ! plot spans this number of columns
Grid1_plot_pad_left(1) = 0.0    ! fraction of full window width for padding on left
Grid1_plot_pad_right(1) = -0.05   ! fraction of full window width for padding on right
Grid1_plot_pad_top(1) = -0.05     ! fraction of full window height for padding at top
Grid1_plot_pad_bot(1) = 0.4     ! fraction of full window height for padding at bottom
Grid1_txt_scale_factor(1) = 0.18 ! multiply txt_scale for subplot by this

Grid1_plot_name(2) = 'Abundance'
Grid1_plot_row(2) = 2           ! number from 1 at top
Grid1_plot_rowspan(2) = 1       ! plot spans this number of rows
Grid1_plot_col(2) =  1          ! number from 1 at left
Grid1_plot_colspan(2) = 1       ! plot spans this number of columns
Grid1_txt_scale_factor(2) = 0.6 ! multiply txt_scale for subplot by this

Grid1_plot_pad_left(2) = -0.02    ! fraction of full window width for padding on left
Grid1_plot_pad_right(2) = 0.06   ! fraction of full window width for padding on right
Grid1_plot_pad_top(2) = 0.15     ! fraction of full window height for padding at top
Grid1_plot_pad_bot(2) = 0.01     ! fraction of full window height for padding at bottom


Grid1_plot_name(3) = 'Mixing'
Grid1_plot_row(3) = 2           ! number from 1 at top
Grid1_plot_rowspan(3) = 1       ! plot spans this number of rows
Grid1_plot_col(3) =  2          ! number from 1 at left
Grid1_plot_colspan(3) = 1       ! plot spans this number of columns
Grid1_txt_scale_factor(3) = 0.6 ! multiply txt_scale for subplot by this

Grid1_plot_pad_left(3) = 0.0    ! fraction of full window width for padding on left
Grid1_plot_pad_right(3) = 0.06   ! fraction of full window width for padding on right
Grid1_plot_pad_top(3) = 0.15     ! fraction of full window height for padding at top
Grid1_plot_pad_bot(3) = 0.01     ! fraction of full window height for padding at bottom

Grid1_plot_name(4) = 'Dynamo'
Grid1_plot_row(4) = 1           ! number from 1 at top
Grid1_plot_rowspan(4) = 1       ! plot spans this number of rows
Grid1_plot_col(4) =  2          ! number from 1 at left
Grid1_plot_colspan(4) = 1       ! plot spans this number of columns

Grid1_plot_pad_left(4) = 0.0    ! fraction of full window width for padding on left
Grid1_plot_pad_right(4) = 0.05   ! fraction of full window width for padding on right
Grid1_plot_pad_top(4) = 0.09     ! fraction of full window height for padding at top
Grid1_plot_pad_bot(4) = -0.03     ! fraction of full window height for padding at bottom
Grid1_txt_scale_factor(4) = 0.5 ! multiply txt_scale for subplot by this


Grid1_plot_name(5) = 'Kipp'
Grid1_plot_row(5) = 1           ! number from 1 at top
Grid1_plot_rowspan(5) = 1       ! plot spans this number of rows
Grid1_plot_col(5) =  1          ! number from 1 at left
Grid1_plot_colspan(5) = 1       ! plot spans this number of columns


Grid1_plot_pad_left(5) = -0.02    ! fraction of full window width for padding on left
Grid1_plot_pad_right(5) = 0.06   ! fraction of full window width for padding on right
Grid1_plot_pad_top(5) = 0.09     ! fraction of full window height for padding at top
Grid1_plot_pad_bot(5) = -0.03     ! fraction of full window height for padding at bottom
Grid1_txt_scale_factor(5) = 0.5 ! multiply txt_scale for subplot by this

Grid1_plot_name(6) = 'History_Panels1' ! 'History_Track1' ! 'Profile_Panels1'
Grid1_plot_row(6) = 1           ! number from 1 at top
Grid1_plot_rowspan(6) = 2       ! plot spans this number of rows
Grid1_plot_col(6) =  3          ! number from 1 at left
Grid1_plot_colspan(6) = 1       ! plot spans this number of columns

Grid1_plot_pad_left(6) = 0.02    ! fraction of full window width for padding on left
Grid1_plot_pad_right(6) = 0.03   ! fraction of full window width for padding on right
Grid1_plot_pad_top(6) = 0.09     ! fraction of full window height for padding at top
Grid1_plot_pad_bot(6) = 0.01     ! fraction of full window height for padding at bottom
Grid1_txt_scale_factor(6) = 0.5 ! multiply txt_scale for subplot by this


!Grid1_plot_name(2) = 'Text_Summary1'
!Grid1_plot_row(2) = 1           ! number from 1 at top
!Grid1_plot_rowspan(2) =1       ! plot spans this number of rows
!Grid1_plot_col(2) =  1          ! number from 1 at left
!Grid1_plot_colspan(2) = 3       ! plot spans this number of columns
!Grid1_plot_pad_left(:) = -0.1    ! fraction of full window width for padding on left
!Grid1_plot_pad_right(:) = -0.05   ! fraction of full window width for padding on right
!Grid1_plot_pad_top(:) = -0.05     ! fraction of full window height for padding at top
!Grid1_plot_pad_bot(:) = 0.35     ! fraction of full window height for padding at bottom
!Grid1_txt_scale_factor(1) = 0.18 ! multiply txt_scale for subplot by this

Grid1_plot_name(4) = 'HR'
Grid1_plot_row(4) = 1           ! number from 1 at top
Grid1_plot_rowspan(4) = 1       ! plot spans this number of rows
Grid1_plot_col(4) =  2          ! number from 1 at left
Grid1_plot_colspan(4) = 1       ! plot spans this number of columns

Grid1_plot_pad_left(4) = 0.0    ! fraction of full window width for padding on left
Grid1_plot_pad_right(4) = 0.06   ! fraction of full window width for padding on right
Grid1_plot_pad_top(4) = 0.09     ! fraction of full window height for padding at top
Grid1_plot_pad_bot(4) = -0.03     ! fraction of full window height for padding at bottom
Grid1_txt_scale_factor(4) = 0.5 ! multiply txt_scale for subplot by this

file_device = 'png'         ! options 'png' and 'vcps' for png and postscript
file_extension = 'png'      ! common names are 'png' and 'ps'

 ! file output
         Grid1_file_flag = .true.
         Grid1_file_dir = 'Grid1'
         Grid1_file_prefix = 'grid1_'
         !Grid1_file_cnt = 1 ! output when mod(model_number,Grid9_file_cnt)==0
         Grid1_file_width = -1 ! (inches) negative means use same value as for window
         Grid1_file_aspect_ratio = -1 ! negative means use same value as for window

!         Grid9_plot_name(3) = 'TRho'
!         Grid9_plot_row(3) = 6 ! number from 1 at top
!         Grid9_plot_rowspan(3) = 3 ! plot spans this number of rows
!         Grid9_plot_col(3) =  2 ! number from 1 at left
!         Grid9_plot_colspan(3) = 1 ! plot spans this number of columns
!         Grid9_plot_pad_left(3) = 0.0267 ! fraction of full window width for padding on left
!         Grid9_plot_pad_right(3) = 0.0867 ! fraction of full window width for padding on right
!         Grid9_plot_pad_top(3) = 0.05 ! fraction of full window height for padding at top
!         Grid9_plot_pad_bot(3) = 0.01 ! fraction of full window height for padding at bottom
!         Grid9_txt_scale_factor(3) = 0.65 ! multiply txt_scale for subplot by this

!         Grid9_plot_name(4) = 'TRho_Profile'
!         Grid9_plot_row(4) = 6 ! number from 1 at top
!         Grid9_plot_rowspan(4) = 3 ! plot spans this number of rows
!         Grid9_plot_col(4) =  3 ! number from 1 at left
!         Grid9_plot_colspan(4) = 1 ! plot spans this number of columns
!         Grid9_plot_pad_left(4) = 0.0533 ! fraction of full window width for padding on left
!         Grid9_plot_pad_right(4) = 0.06 ! fraction of full window width for padding on right
!         Grid9_plot_pad_top(4) = 0.05 ! fraction of full window height for padding at top
!         Grid9_plot_pad_bot(4) = 0.01 ! fraction of full window height for padding at bottom
!         Grid9_txt_scale_factor(4) = 0.7 ! multiply txt_scale for subplot by this


  !# Network window
      ! Shows N vs Z for isotopes in current net

         Network_win_flag = .false.

         Network_win_width = 6
         Network_win_aspect_ratio = 0.75 ! aspect_ratio = height/width

         Network_xleft = 0.15
         Network_xright = 0.85
         Network_ybot = 0.15
         Network_ytop = 0.85
         Network_txt_scale = 1.0
         Network_title = 'Network'

         ! axis limits -- to override system default selections
         Network_nmin = -101d0 ! only used if /= -101d0
         Network_nmax = -101d0 ! only used if /= -101d0
         Network_zmin = -101d0 ! only used if /= -101d0
         Network_zmax = -101d0 ! only used if /= -101d0

         ! Show mass fraction as a coloured square
         Network_show_mass_fraction = .true.
         ! Limits on mass fractions to show
         Network_log_mass_frac_min = -5.0d0
         Network_log_mass_frac_max = 0.0d0

         ! Label Y axis with element name
         Network_show_element_names = .true.

         ! Enables calling a subroutine to add extra information to a plot
         ! see `$MESA_DIR/star/other/pgstar_decorator.f90`
         Network_use_decorator = .false.

         ! Add colorbar
         Network_show_colorbar = .true.

         ! file output
         Network_file_flag = .false.
         Network_file_dir = 'png'
         Network_file_prefix = 'Network_'
         Network_file_interval = 5 ! output when `mod(model_number,Network_file_interval)==0`
         Network_file_width = -1 ! (inches) negative means use same value as for window
         Network_file_aspect_ratio = -1 ! negative means use same value as for window



      !# History Tracks

         !### History_Track1

            History_Track1_win_flag = .false.
            History_Track1_win_width = 6
            History_Track1_win_aspect_ratio = 0.75 ! aspect_ratio = height/width

            History_Track1_xleft = 0.15
            History_Track1_xright = 0.85
            History_Track1_ybot = 0.15
            History_Track1_ytop = 0.85
            History_Track1_txt_scale = 1.0
            History_Track1_title = 'History_Track1'

            ! set default
            History_Track1_xname = 'log_L'
            History_Track1_yname = 'surface_c12'
            History_Track1_xaxis_label = 'log L/L\d\(2281)'
            History_Track1_yaxis_label = 'c12'
            History_Track1_reverse_xaxis = .false.
            History_Track1_reverse_yaxis = .false.
            History_Track1_log_xaxis = .false. ! show log10 of abs value
            History_Track1_log_yaxis = .true. ! show log10 of abs value

            History_Track1_xmin = -101d0 ! only used if /= -101d0
            History_Track1_xmax = -101d0 ! only used if /= -101d0
            History_Track1_ymin = -101d0 ! only used if /= -101d0
            History_Track1_ymax = -101d0 ! only used if /= -101d0

            History_Track1_xmargin = 0.1
            History_Track1_ymargin = 0.1
            History_Track1_dxmin = -1
            History_Track1_dymin = -1

            History_Track1_step_min = -1 ! only plot models with model number >= this
            History_Track1_step_max = 999999 ! only plot models with model number <= this

            show_History_Track1_target_box = .false.
            History_Track1_n_sigma = -3 ! -n means show sig 1..n
            History_Track1_xtarget = 0
            History_Track1_xsigma = 0
            History_Track1_ytarget = 0
            History_Track1_ysigma = 0

            show_History_Track1_annotation1 = .false.
            show_History_Track1_annotation2 = .false.
            show_History_Track1_annotation3 = .false.

            History_Track1_fname = '' ! file name for extra track data

            ! Enables calling a subroutine to add extra information to a plot
            ! see `$MESA_DIR/star/other/pgstar_decorator.f90`
             History_Track1_use_decorator = .false.

            ! file output
            History_Track1_file_flag = .false.
            History_Track1_file_dir = 'png'
            History_Track1_file_prefix = 'track1_'
            History_Track1_file_interval = 5 ! output when `mod(model_number,History_Track1_file_interval)==0`
            History_Track1_file_width = -1 ! (inches) negative means use same value as for window
            History_Track1_file_aspect_ratio = -1 ! negative means use same value as for window



            !# History Panels

               !### History_Panels1

                  History_Panels1_win_flag = .false.

                  History_Panels1_win_width = 6
                  History_Panels1_win_aspect_ratio = 0.75 ! aspect_ratio = height/width

                  History_Panels1_xleft = 0.15
                  History_Panels1_xright = 0.85
                  History_Panels1_ybot = 0.15
                  History_Panels1_ytop = 0.85
                  History_Panels1_txt_scale = 1.0
                  History_Panels1_title = 'History_Panels1'

                  History_Panels1_xaxis_name = 'log_L'
                  History_Panels1_xmin = -101d0
                  History_Panels1_xmax = -101d0
                  History_Panels1_max_width = 100 ! only used if > 0.  causes xmin to move with xmax.
                  History_Panels1_dxmin = -1
                  History_Panels1_xaxis_reversed = .false.
                  History_Panels1_xaxis_log = .false. ! show log10 of abs value
                  History_Panels1_xmargin = 0.0

                  History_Panels1_yaxis_name(:) = 'surface_c12'
                  History_Panels1_yaxis_reversed(:) = .false.
                  History_Panels1_yaxis_log(:) = .true. ! show log10 of abs value
                  History_Panels1_ymin(:) = -101d0 ! only used if /= -101d0
                  History_Panels1_ymax(:) = -101d0 ! only used if /= -101d0
                  History_Panels1_ymargin(:) = 0.1
                  History_Panels1_dymin(:) = -1

                  History_Panels1_other_yaxis_name(:) = 'surface_li7'
                  History_Panels1_other_yaxis_reversed(:) = .false.
                  History_Panels1_other_yaxis_log(:) = .true. ! show log10 of abs value
                  History_Panels1_other_ymin(:) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_ymax(:) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_ymargin(:) = 0.1
                  History_Panels1_other_dymin(:) = -1

                  History_Panels1_points_name(:) = ''

                  ! setup default
                  History_Panels1_num_panels = 2

                  History_Panels1_yaxis_name(1) = 'surface_c12'
                  History_Panels1_yaxis_reversed(1) = .false.
                  History_Panels1_yaxis_log(1) = .true.
                  History_Panels1_ymin(1) = -101d0 ! only used if /= -101d0
                  History_Panels1_ymax(1) = -101d0 ! only used if /= -101d0
                  History_Panels1_dymin(1) = -1

                  History_Panels1_other_yaxis_name(1) = 'surface_c13'
                  History_Panels1_other_yaxis_reversed(1) = .false.
                  History_Panels1_other_yaxis_log(1) = .true.
                  History_Panels1_other_ymin(1) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_ymax(1) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_dymin(1) = -1

                  History_Panels1_yaxis_name(2) = 'surface_li7'
                  History_Panels1_yaxis_reversed(2) = .false.
                  History_Panels1_yaxis_log(2) = .true.
                  History_Panels1_ymin(2) = -101d0 ! only used if /= -101d0
                  History_Panels1_ymax(2) = -101d0 ! only used if /= -101d0
                  History_Panels1_dymin(2) = -1

                  History_Panels1_other_yaxis_name(2) = 'surface_he3'
                  History_Panels1_other_yaxis_reversed(2) = .false.
                  History_Panels1_other_yaxis_log(2) = .true.
                  History_Panels1_other_ymin(2) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_ymax(2) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_dymin(2) = -1

                  History_Panels1_yaxis_name(3) = 'star_mass'
                  History_Panels1_yaxis_reversed(3) = .false.
                  History_Panels1_ymin(3) = -101d0 ! only used if /= -101d0
                  History_Panels1_ymax(3) = -101d0 ! only used if /= -101d0
                  History_Panels1_dymin(3) = -1

                  History_Panels1_other_yaxis_name(3) = 'log_abs_mdot'
                  History_Panels1_other_yaxis_reversed(3) = .false.
                  History_Panels1_other_ymin(3) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_ymax(3) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_dymin(3) = -1

                  ! Enables calling a subroutine to add extra information to a plot
                  ! see `$MESA_DIR/star/other/pgstar_decorator.f90`
                  History_Panels1_use_decorator = .false.

                  ! file output
                  History_Panels1_file_flag = .false.
                  History_Panels1_file_dir = 'png'
                  History_Panels1_file_prefix = 'History_Panels1_'
                  History_Panels1_file_interval = 5 ! output when `mod(model_number,History_Panels1_file_interval)==0`
                  History_Panels1_file_width = -1 ! (inches) negative means use same value as for window
                  History_Panels1_file_aspect_ratio = -1 ! negative means use same value as for window




                  !### Profile_Panels1

                     Profile_Panels1_win_flag = .true.

                     Profile_Panels1_win_width = 8
                     Profile_Panels1_win_aspect_ratio = 1.25 ! aspect_ratio = height/width

                     Profile_Panels1_xleft = 0.15
                     Profile_Panels1_xright = 0.83
                     Profile_Panels1_ybot = 0.15
                     Profile_Panels1_ytop = 0.9
                     Profile_Panels1_txt_scale = 1.0
                     Profile_Panels1_title = 'Profile Panels1'

                     Profile_Panels1_xaxis_name = 'mass'
                     Profile_Panels1_xaxis_reversed = .false.
                     Profile_Panels1_xmin = 0.22 ! only used if /= -101d0
                     Profile_Panels1_xmax = 0.28 ! only used if /= -101d0
                     Profile_Panels1_xmargin = 0d0
                     Profile_Panels1_show_mix_regions_on_xaxis = .false.

                     Profile_Panels1_yaxis_name(:) = 'Prandtl'
                     Profile_Panels1_yaxis_reversed(:) = .false.
                     Profile_Panels1_yaxis_log(:) = .false. ! show log10 of abs value
                     Profile_Panels1_ymin(2) =  1.337 ! only used if /= -101d0
                     Profile_Panels1_ymax(2) =  1.339 ! only used if /= -101d0
                     Profile_Panels1_ycenter(:) = -101d0 ! only used if /= -101d0
                     Profile_Panels1_ymargin(:) = 0.1
                     Profile_Panels1_dymin(:) = -1

                     Profile_Panels1_other_yaxis_name(:) = ''
                     Profile_Panels1_other_yaxis_reversed(:) = .false.
                     Profile_Panels1_other_yaxis_log(:) = .false. ! show log10 of abs value
                     Profile_Panels1_other_ymin(:) = -101d0 ! only used if /= -101d0
                     Profile_Panels1_other_ymax(:) = -101d0 ! only used if /= -101d0
                     Profile_Panels1_other_ycenter(:) = -101d0 ! only used if /= -101d0
                     Profile_Panels1_other_ymargin(:) = 0.1
                     Profile_Panels1_other_dymin(:) = -1

                     Profile_Panels1_show_grid = .false.

                     ! setup default plot
                     Profile_Panels1_num_panels = 3
                     Profile_Panels1_yaxis_name(1) = 'logT'
                     Profile_Panels1_other_yaxis_name(1) = 'Prandtl'
                     Profile_Panels1_yaxis_name(2) = 'mu'
                     Profile_Panels1_other_yaxis_name(2) = 'he3'!'he3'


                     Profile_Panels1_yaxis_name(3) = 'gradr_sub_grada' !'super_ad'
                     Profile_Panels1_other_yaxis_name(3) = 'gradL_composition_term'!'he3'

                     ! Enables calling a subroutine to add extra information to a plot
                     ! see `$MESA_DIR/star/other/pgstar_decorator.f90`
                     Profile_Panels1_use_decorator = .false.

                     ! file output
                     Profile_Panels1_file_flag = .false.
                     Profile_Panels1_file_dir = 'png'
                     Profile_Panels1_file_prefix = 'profile_panels1_'
                     Profile_Panels1_file_interval = 5 ! output when `mod(model_number,Profile_Panels1_file_interval)==0`
                     Profile_Panels1_file_width = -1 ! (inches) negative means use same value as for window
                     Profile_Panels1_file_aspect_ratio = -1 ! negative means use same value as for window

/ ! end of pgstar namelist



==> mesa_models/template_work_thermohaline/inlist_pgstar_thermohaline <==
&pgstar

pgstar_show_age_in_years = .false.
pgstar_show_age_in_seconds = .true.

! Kippenhahn diagram history plot

Kipp_win_flag = .true.

! window properties
Kipp_win_width = 9
Kipp_win_aspect_ratio = 0.74
Kipp_title = 'Kippenhahn'

! y axis limits
Kipp_mass_max = 0.4
Kipp_mass_min = 0.22
Kipp_show_mass_boundaries = .true.
Kipp_xaxis_name='model_number'

! x axis limits
!Kipp_xmax = -1              ! maximum step number.  negative means use default.
!Kipp_xmin = -1            ! minimum step number.  negative means use default.
!Kipp_max_width = -1         ! only used if > 0.  causes xmin to move with xmax.

! file output
Kipp_file_flag = .false.
Kipp_file_dir = 'Kipp'
Kipp_file_prefix = 'kipp_'
!Kipp_file_cnt = 1          ! output when mod(model_number,Kipp_file_cnt)==0
Kipp_file_width = -1        ! (inches) negative means use same value as for window
Kipp_file_aspect_ratio = -1 ! negative means use same value as for window
file_device = 'png'         ! options 'png' and 'vcps' for png and postscript
file_extension = 'png'      ! common names are 'png' and 'ps'


!--------------------------------------------------------------------------------------


! Abundance profile plot

Abundance_win_flag = .true.


! isotopes to plot
Abundance_num_isos_to_show = 2
Abundance_which_isos_to_show(1) = 'h1'
Abundance_which_isos_to_show(2) = 'he3'


! window properties
Abundance_win_width =
Abundance_win_aspect_ratio =

Abundance_xleft =
Abundance_xright =
Abundance_ybot =
Abundance_ytop =
Abundance_txt_scale =
Abundance_title =

! isotopes to plot
Abundance_num_isos_to_show = 8
Abundance_which_isos_to_show(1) = 'h1'
Abundance_which_isos_to_show(2) = 'he3'
Abundance_which_isos_to_show(3) = 'c12'
Abundance_which_isos_to_show(4) = 'o16'
Abundance_which_isos_to_show(5) = 'n14'
Abundance_which_isos_to_show(6) = 'c13'
Abundance_which_isos_to_show(7) = 'he4'
Abundance_which_isos_to_show(8) = 'Li7'

! number and size of isotope labels along curves
num_abundance_line_labels =
Abundance_line_txt_scale_factor =

! number and size of isotopes on legend
Abundance_legend_max_cnt = 0
Abundance_legend_txt_scale_factor =

! xaxis name and orientation
Abundance_xaxis_name =
Abundance_xaxis_reversed =

! xaxis limits
Abundance_xmin = 0.2
Abundance_xmax = 0.4

! yaxis limits
Abundance_log_mass_frac_min = -3
Abundance_log_mass_frac_max = 0.1

!------------------------------------------------------------------------------------

! Profile Panel





Profile_Panels1_num_panels = 3
Profile_Panels1_txt_scale = 1.0
Profile_Panels1_title = 'Diagnostic'
Profile_Panels1_win_flag = .true.
Profile_Panels1_xaxis_name = 'logtau' !'logT'
Profile_Panels1_xmin = -0.6 !4 ! only used if /= -101d0
Profile_Panels1_xmax = 10   ! only used if /= -101d0
Profile_Panels1_yaxis_name(:) = 'opacity'
Profile_Panels1_ymin(:) = -101! only used if /= -101d0
Profile_Panels1_ymax(:) = -101 ! only used if /= -101d0
Profile_Panels1_other_yaxis_name(:) = 'logRho'
Profile_Panels1_other_ymin(:) = -101 ! only used if /= -101d0
Profile_Panels1_other_ymax(:) = -101 ! only used if /= -101d0
Profile_Panels1_show_grid = .true.
Profile_Panels1_xaxis_reversed = .false.

Profile_Panels1_yaxis_name(2) = 'entropy' !'entropy'
Profile_Panels1_other_yaxis_name(2) = 'extra_heat' !mass'
Profile_Panels1_ymin(2) = !14! only used if /= -101d0
Profile_Panels1_ymax(2) = !19 ! only used if /= -101d0
Profile_Panels1_other_ymin(2) = !14
Profile_Panels1_other_ymax(2) = !19
Profile_Panels1_yaxis_name(3) = 'logT' ! pgas_div_ptotal' ! 'logtau'
Profile_Panels1_other_yaxis_name(3) = 'log_L_div_Ledd' !'log_L_div_Ledd'


! ----------------------

pgstar_lw = 6 ! integer

! ----------------------


! Mixing profile

Mixing_win_flag = .true.

! window properties
Mixing_win_width =
Mixing_win_aspect_ratio =
Mixing_title = 'Mixing'

! x-axis
Mixing_xaxis_name = 'mass'
Mixing_xaxis_reversed = .false.
Mixing_xmin =  0.24
Mixing_xmax =  0.5

! y-axis
Mixing_ymin = 0
Mixing_ymax = 18
Mixing_dymin =

! file output
Mixing_file_flag = .false.
Mixing_file_dir = 'Mixing'
Mixing_file_prefix = 'mixing_'
!Mixing_file_cnt = 5           ! output when mod(model_number,Mixing_file_cnt)==0
Mixing_file_width = -1        ! (inches) negative means use same value as for window
Mixing_file_aspect_ratio = -1 ! negative means use same value as for window
file_device = 'png'         ! options 'png' and 'vcps' for png and postscript respectively
file_extension = 'png'      ! common names are 'png' and 'ps'

! ---------------------

  !### Profile_Panels4

         Profile_Panels4_win_flag = .true.
         Profile_Panels4_win_width = 6
         Profile_Panels4_show_grid = .false.

         ! setup default plot
         Profile_Panels4_win_aspect_ratio = 0.75
         !Profile_Panels4_txt_scale = 0.9
         Profile_Panels4_ybot = 0.1
         Profile_Panels4_ytop = 0.9
         Profile_Panels4_title = 'Dynamo'

         Profile_Panels4_xaxis_name = 'radius_cm'
         Profile_Panels4_xmin = 2.5d8 ! only used if /= -101d0
         Profile_Panels4_xmax = 3.85d8 ! only used if /= -101d0



         Profile_Panels4_num_panels = 1
         Profile_Panels4_yaxis_name(1) = 'Dynamo'
         !Profile_Panels4_yaxis_name(2) = 'Power'
         !Profile_Panels4_yaxis_name(3) = 'Mixing'
         !Profile_Panels4_yaxis_name(4) = 'Dynamo'

         ! file output
         Profile_Panels4_file_flag = .false.
         Profile_Panels4_file_dir = 'png'
         Profile_Panels4_file_prefix = 'profile_Panels4_'
        ! Profile_Panels4_file_cnt = 5 ! output when mod(model_number,Profile_Panels4_file_cnt)==0
         Profile_Panels4_file_width = -1 ! (inches) negative means use same value as for window
         Profile_Panels4_file_aspect_ratio = -1 ! negative means use same value as for window


!------------ Text_Summary windows

Text_Summary1_win_flag = .true.
Text_Summary1_win_width = 5
Text_Summary1_win_aspect_ratio = 0.13

Text_Summary1_xleft = 0.06
Text_Summary1_xright = 1.02
Text_Summary1_ybot = 0.0
Text_Summary1_ytop = 1.0
Text_Summary1_txt_scale = 4.0
Text_Summary1_title = ''

Text_Summary1_num_rows = 3 ! <= 20
Text_Summary1_num_cols = 4 ! <= 20
Text_Summary1_name(:,:) = ''

Text_Summary1_name(1,1) = 'time_step'
Text_Summary1_name(1,2) = 'num_zones'
Text_Summary1_name(1,3) = 'star_mass'
Text_Summary1_name(1,4) = 'star_mdot'

Text_Summary1_name(2,1) = 'log_total_angular_momentum'
Text_Summary1_name(2,2) = 'center_omega'
Text_Summary1_name(2,3) = 'surf_avg_omega'
Text_Summary1_name(2,4) = 'surf_avg_v_rot'

Text_Summary1_name(3,1) = 'log_Teff'
Text_Summary1_name(3,2) = 'photosphere_L'
Text_Summary1_name(3,3) = 'photosphere_r'
Text_Summary1_name(3,4) = 'star_age'


!------------------------------------------------------------------------------------


Kipp_win_flag = .false.
Abundance_win_flag = .false.
Profile_Panels1_win_flag = .false.
Profile_Panels4_win_flag = .false.
Mixing_win_flag = .false.
Dynamo_win_flag = .false.
Text_Summary1_win_flag = .false.

!------------------------------------------------------------------------------------

Grid1_win_flag = .true.
Grid1_win_width = 12
Grid1_win_aspect_ratio = 0.65

Grid1_num_cols = 3 ! divide plotting region into this many equal width cols
Grid1_num_rows = 2 ! divide plotting region into this many equal height rows
Grid1_num_plots = 6 ! <= 10

Grid1_xleft = 0.07 ! fraction of full window width for margin on left
Grid1_xright = 0.98 ! fraction of full window width for margin on right
Grid1_ybot = 0.05 ! fraction of full window width for margin on bottom
Grid1_ytop = 0.92 ! fraction of full window width for margin on top


Grid1_plot_name(1) = 'Text_Summary1'
Grid1_plot_row(1) = 1           ! number from 1 at top
Grid1_plot_rowspan(1) =1       ! plot spans this number of rows
Grid1_plot_col(1) =  1          ! number from 1 at left
Grid1_plot_colspan(1) = 3       ! plot spans this number of columns
Grid1_plot_pad_left(1) = 0.0    ! fraction of full window width for padding on left
Grid1_plot_pad_right(1) = -0.05   ! fraction of full window width for padding on right
Grid1_plot_pad_top(1) = -0.05     ! fraction of full window height for padding at top
Grid1_plot_pad_bot(1) = 0.4     ! fraction of full window height for padding at bottom
Grid1_txt_scale_factor(1) = 0.18 ! multiply txt_scale for subplot by this

Grid1_plot_name(2) = 'Abundance'
Grid1_plot_row(2) = 2           ! number from 1 at top
Grid1_plot_rowspan(2) = 1       ! plot spans this number of rows
Grid1_plot_col(2) =  1          ! number from 1 at left
Grid1_plot_colspan(2) = 1       ! plot spans this number of columns
Grid1_txt_scale_factor(2) = 0.6 ! multiply txt_scale for subplot by this

Grid1_plot_pad_left(2) = -0.02    ! fraction of full window width for padding on left
Grid1_plot_pad_right(2) = 0.06   ! fraction of full window width for padding on right
Grid1_plot_pad_top(2) = 0.15     ! fraction of full window height for padding at top
Grid1_plot_pad_bot(2) = 0.01     ! fraction of full window height for padding at bottom


Grid1_plot_name(3) = 'Mixing'
Grid1_plot_row(3) = 2           ! number from 1 at top
Grid1_plot_rowspan(3) = 1       ! plot spans this number of rows
Grid1_plot_col(3) =  2          ! number from 1 at left
Grid1_plot_colspan(3) = 1       ! plot spans this number of columns
Grid1_txt_scale_factor(3) = 0.6 ! multiply txt_scale for subplot by this

Grid1_plot_pad_left(3) = 0.0    ! fraction of full window width for padding on left
Grid1_plot_pad_right(3) = 0.06   ! fraction of full window width for padding on right
Grid1_plot_pad_top(3) = 0.15     ! fraction of full window height for padding at top
Grid1_plot_pad_bot(3) = 0.01     ! fraction of full window height for padding at bottom

Grid1_plot_name(4) = 'Dynamo'
Grid1_plot_row(4) = 1           ! number from 1 at top
Grid1_plot_rowspan(4) = 1       ! plot spans this number of rows
Grid1_plot_col(4) =  2          ! number from 1 at left
Grid1_plot_colspan(4) = 1       ! plot spans this number of columns

Grid1_plot_pad_left(4) = 0.0    ! fraction of full window width for padding on left
Grid1_plot_pad_right(4) = 0.05   ! fraction of full window width for padding on right
Grid1_plot_pad_top(4) = 0.09     ! fraction of full window height for padding at top
Grid1_plot_pad_bot(4) = -0.03     ! fraction of full window height for padding at bottom
Grid1_txt_scale_factor(4) = 0.5 ! multiply txt_scale for subplot by this


Grid1_plot_name(5) = 'Kipp'
Grid1_plot_row(5) = 1           ! number from 1 at top
Grid1_plot_rowspan(5) = 1       ! plot spans this number of rows
Grid1_plot_col(5) =  1          ! number from 1 at left
Grid1_plot_colspan(5) = 1       ! plot spans this number of columns


Grid1_plot_pad_left(5) = -0.02    ! fraction of full window width for padding on left
Grid1_plot_pad_right(5) = 0.06   ! fraction of full window width for padding on right
Grid1_plot_pad_top(5) = 0.09     ! fraction of full window height for padding at top
Grid1_plot_pad_bot(5) = -0.03     ! fraction of full window height for padding at bottom
Grid1_txt_scale_factor(5) = 0.5 ! multiply txt_scale for subplot by this

Grid1_plot_name(6) = 'History_Panels1' ! 'History_Track1' ! 'Profile_Panels1'
Grid1_plot_row(6) = 1           ! number from 1 at top
Grid1_plot_rowspan(6) = 2       ! plot spans this number of rows
Grid1_plot_col(6) =  3          ! number from 1 at left
Grid1_plot_colspan(6) = 1       ! plot spans this number of columns

Grid1_plot_pad_left(6) = 0.02    ! fraction of full window width for padding on left
Grid1_plot_pad_right(6) = 0.03   ! fraction of full window width for padding on right
Grid1_plot_pad_top(6) = 0.09     ! fraction of full window height for padding at top
Grid1_plot_pad_bot(6) = 0.01     ! fraction of full window height for padding at bottom
Grid1_txt_scale_factor(6) = 0.5 ! multiply txt_scale for subplot by this


!Grid1_plot_name(2) = 'Text_Summary1'
!Grid1_plot_row(2) = 1           ! number from 1 at top
!Grid1_plot_rowspan(2) =1       ! plot spans this number of rows
!Grid1_plot_col(2) =  1          ! number from 1 at left
!Grid1_plot_colspan(2) = 3       ! plot spans this number of columns
!Grid1_plot_pad_left(:) = -0.1    ! fraction of full window width for padding on left
!Grid1_plot_pad_right(:) = -0.05   ! fraction of full window width for padding on right
!Grid1_plot_pad_top(:) = -0.05     ! fraction of full window height for padding at top
!Grid1_plot_pad_bot(:) = 0.35     ! fraction of full window height for padding at bottom
!Grid1_txt_scale_factor(1) = 0.18 ! multiply txt_scale for subplot by this

Grid1_plot_name(4) = 'HR'
Grid1_plot_row(4) = 1           ! number from 1 at top
Grid1_plot_rowspan(4) = 1       ! plot spans this number of rows
Grid1_plot_col(4) =  2          ! number from 1 at left
Grid1_plot_colspan(4) = 1       ! plot spans this number of columns

Grid1_plot_pad_left(4) = 0.0    ! fraction of full window width for padding on left
Grid1_plot_pad_right(4) = 0.06   ! fraction of full window width for padding on right
Grid1_plot_pad_top(4) = 0.09     ! fraction of full window height for padding at top
Grid1_plot_pad_bot(4) = -0.03     ! fraction of full window height for padding at bottom
Grid1_txt_scale_factor(4) = 0.5 ! multiply txt_scale for subplot by this

file_device = 'png'         ! options 'png' and 'vcps' for png and postscript
file_extension = 'png'      ! common names are 'png' and 'ps'

 ! file output
         Grid1_file_flag = .true.
         Grid1_file_dir = 'Grid1'
         Grid1_file_prefix = 'grid1_'
         !Grid1_file_cnt = 1 ! output when mod(model_number,Grid9_file_cnt)==0
         Grid1_file_width = -1 ! (inches) negative means use same value as for window
         Grid1_file_aspect_ratio = -1 ! negative means use same value as for window

!         Grid9_plot_name(3) = 'TRho'
!         Grid9_plot_row(3) = 6 ! number from 1 at top
!         Grid9_plot_rowspan(3) = 3 ! plot spans this number of rows
!         Grid9_plot_col(3) =  2 ! number from 1 at left
!         Grid9_plot_colspan(3) = 1 ! plot spans this number of columns
!         Grid9_plot_pad_left(3) = 0.0267 ! fraction of full window width for padding on left
!         Grid9_plot_pad_right(3) = 0.0867 ! fraction of full window width for padding on right
!         Grid9_plot_pad_top(3) = 0.05 ! fraction of full window height for padding at top
!         Grid9_plot_pad_bot(3) = 0.01 ! fraction of full window height for padding at bottom
!         Grid9_txt_scale_factor(3) = 0.65 ! multiply txt_scale for subplot by this

!         Grid9_plot_name(4) = 'TRho_Profile'
!         Grid9_plot_row(4) = 6 ! number from 1 at top
!         Grid9_plot_rowspan(4) = 3 ! plot spans this number of rows
!         Grid9_plot_col(4) =  3 ! number from 1 at left
!         Grid9_plot_colspan(4) = 1 ! plot spans this number of columns
!         Grid9_plot_pad_left(4) = 0.0533 ! fraction of full window width for padding on left
!         Grid9_plot_pad_right(4) = 0.06 ! fraction of full window width for padding on right
!         Grid9_plot_pad_top(4) = 0.05 ! fraction of full window height for padding at top
!         Grid9_plot_pad_bot(4) = 0.01 ! fraction of full window height for padding at bottom
!         Grid9_txt_scale_factor(4) = 0.7 ! multiply txt_scale for subplot by this


  !# Network window
      ! Shows N vs Z for isotopes in current net

         Network_win_flag = .false.

         Network_win_width = 6
         Network_win_aspect_ratio = 0.75 ! aspect_ratio = height/width

         Network_xleft = 0.15
         Network_xright = 0.85
         Network_ybot = 0.15
         Network_ytop = 0.85
         Network_txt_scale = 1.0
         Network_title = 'Network'

         ! axis limits -- to override system default selections
         Network_nmin = -101d0 ! only used if /= -101d0
         Network_nmax = -101d0 ! only used if /= -101d0
         Network_zmin = -101d0 ! only used if /= -101d0
         Network_zmax = -101d0 ! only used if /= -101d0

         ! Show mass fraction as a coloured square
         Network_show_mass_fraction = .true.
         ! Limits on mass fractions to show
         Network_log_mass_frac_min = -5.0d0
         Network_log_mass_frac_max = 0.0d0

         ! Label Y axis with element name
         Network_show_element_names = .true.

         ! Enables calling a subroutine to add extra information to a plot
         ! see `$MESA_DIR/star/other/pgstar_decorator.f90`
         Network_use_decorator = .false.

         ! Add colorbar
         Network_show_colorbar = .true.

         ! file output
         Network_file_flag = .false.
         Network_file_dir = 'png'
         Network_file_prefix = 'Network_'
         Network_file_interval = 5 ! output when `mod(model_number,Network_file_interval)==0`
         Network_file_width = -1 ! (inches) negative means use same value as for window
         Network_file_aspect_ratio = -1 ! negative means use same value as for window



      !# History Tracks

         !### History_Track1

            History_Track1_win_flag = .false.
            History_Track1_win_width = 6
            History_Track1_win_aspect_ratio = 0.75 ! aspect_ratio = height/width

            History_Track1_xleft = 0.15
            History_Track1_xright = 0.85
            History_Track1_ybot = 0.15
            History_Track1_ytop = 0.85
            History_Track1_txt_scale = 1.0
            History_Track1_title = 'History_Track1'

            ! set default
            History_Track1_xname = 'log_L'
            History_Track1_yname = 'surface_c12'
            History_Track1_xaxis_label = 'log L/L\d\(2281)'
            History_Track1_yaxis_label = 'c12'
            History_Track1_reverse_xaxis = .false.
            History_Track1_reverse_yaxis = .false.
            History_Track1_log_xaxis = .false. ! show log10 of abs value
            History_Track1_log_yaxis = .true. ! show log10 of abs value

            History_Track1_xmin = -101d0 ! only used if /= -101d0
            History_Track1_xmax = -101d0 ! only used if /= -101d0
            History_Track1_ymin = -101d0 ! only used if /= -101d0
            History_Track1_ymax = -101d0 ! only used if /= -101d0

            History_Track1_xmargin = 0.1
            History_Track1_ymargin = 0.1
            History_Track1_dxmin = -1
            History_Track1_dymin = -1

            History_Track1_step_min = -1 ! only plot models with model number >= this
            History_Track1_step_max = 999999 ! only plot models with model number <= this

            show_History_Track1_target_box = .false.
            History_Track1_n_sigma = -3 ! -n means show sig 1..n
            History_Track1_xtarget = 0
            History_Track1_xsigma = 0
            History_Track1_ytarget = 0
            History_Track1_ysigma = 0

            show_History_Track1_annotation1 = .false.
            show_History_Track1_annotation2 = .false.
            show_History_Track1_annotation3 = .false.

            History_Track1_fname = '' ! file name for extra track data

            ! Enables calling a subroutine to add extra information to a plot
            ! see `$MESA_DIR/star/other/pgstar_decorator.f90`
             History_Track1_use_decorator = .false.

            ! file output
            History_Track1_file_flag = .false.
            History_Track1_file_dir = 'png'
            History_Track1_file_prefix = 'track1_'
            History_Track1_file_interval = 5 ! output when `mod(model_number,History_Track1_file_interval)==0`
            History_Track1_file_width = -1 ! (inches) negative means use same value as for window
            History_Track1_file_aspect_ratio = -1 ! negative means use same value as for window



            !# History Panels

               !### History_Panels1

                  History_Panels1_win_flag = .false.

                  History_Panels1_win_width = 6
                  History_Panels1_win_aspect_ratio = 0.75 ! aspect_ratio = height/width

                  History_Panels1_xleft = 0.15
                  History_Panels1_xright = 0.85
                  History_Panels1_ybot = 0.15
                  History_Panels1_ytop = 0.85
                  History_Panels1_txt_scale = 1.0
                  History_Panels1_title = 'History_Panels1'

                  History_Panels1_xaxis_name = 'log_L'
                  History_Panels1_xmin = -101d0
                  History_Panels1_xmax = -101d0
                  History_Panels1_max_width = 100 ! only used if > 0.  causes xmin to move with xmax.
                  History_Panels1_dxmin = -1
                  History_Panels1_xaxis_reversed = .false.
                  History_Panels1_xaxis_log = .false. ! show log10 of abs value
                  History_Panels1_xmargin = 0.0

                  History_Panels1_yaxis_name(:) = 'surface_c12'
                  History_Panels1_yaxis_reversed(:) = .false.
                  History_Panels1_yaxis_log(:) = .true. ! show log10 of abs value
                  History_Panels1_ymin(:) = -101d0 ! only used if /= -101d0
                  History_Panels1_ymax(:) = -101d0 ! only used if /= -101d0
                  History_Panels1_ymargin(:) = 0.1
                  History_Panels1_dymin(:) = -1

                  History_Panels1_other_yaxis_name(:) = 'surface_li7'
                  History_Panels1_other_yaxis_reversed(:) = .false.
                  History_Panels1_other_yaxis_log(:) = .true. ! show log10 of abs value
                  History_Panels1_other_ymin(:) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_ymax(:) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_ymargin(:) = 0.1
                  History_Panels1_other_dymin(:) = -1

                  History_Panels1_points_name(:) = ''

                  ! setup default
                  History_Panels1_num_panels = 2

                  History_Panels1_yaxis_name(1) = 'surface_c12'
                  History_Panels1_yaxis_reversed(1) = .false.
                  History_Panels1_yaxis_log(1) = .true.
                  History_Panels1_ymin(1) = -101d0 ! only used if /= -101d0
                  History_Panels1_ymax(1) = -101d0 ! only used if /= -101d0
                  History_Panels1_dymin(1) = -1

                  History_Panels1_other_yaxis_name(1) = 'surface_c13'
                  History_Panels1_other_yaxis_reversed(1) = .false.
                  History_Panels1_other_yaxis_log(1) = .true.
                  History_Panels1_other_ymin(1) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_ymax(1) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_dymin(1) = -1

                  History_Panels1_yaxis_name(2) = 'surface_li7'
                  History_Panels1_yaxis_reversed(2) = .false.
                  History_Panels1_yaxis_log(2) = .true.
                  History_Panels1_ymin(2) = -101d0 ! only used if /= -101d0
                  History_Panels1_ymax(2) = -101d0 ! only used if /= -101d0
                  History_Panels1_dymin(2) = -1

                  History_Panels1_other_yaxis_name(2) = 'surface_he3'
                  History_Panels1_other_yaxis_reversed(2) = .false.
                  History_Panels1_other_yaxis_log(2) = .true.
                  History_Panels1_other_ymin(2) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_ymax(2) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_dymin(2) = -1

                  History_Panels1_yaxis_name(3) = 'star_mass'
                  History_Panels1_yaxis_reversed(3) = .false.
                  History_Panels1_ymin(3) = -101d0 ! only used if /= -101d0
                  History_Panels1_ymax(3) = -101d0 ! only used if /= -101d0
                  History_Panels1_dymin(3) = -1

                  History_Panels1_other_yaxis_name(3) = 'log_abs_mdot'
                  History_Panels1_other_yaxis_reversed(3) = .false.
                  History_Panels1_other_ymin(3) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_ymax(3) = -101d0 ! only used if /= -101d0
                  History_Panels1_other_dymin(3) = -1

                  ! Enables calling a subroutine to add extra information to a plot
                  ! see `$MESA_DIR/star/other/pgstar_decorator.f90`
                  History_Panels1_use_decorator = .false.

                  ! file output
                  History_Panels1_file_flag = .false.
                  History_Panels1_file_dir = 'png'
                  History_Panels1_file_prefix = 'History_Panels1_'
                  History_Panels1_file_interval = 5 ! output when `mod(model_number,History_Panels1_file_interval)==0`
                  History_Panels1_file_width = -1 ! (inches) negative means use same value as for window
                  History_Panels1_file_aspect_ratio = -1 ! negative means use same value as for window




                  !### Profile_Panels1

                     Profile_Panels1_win_flag = .true.

                     Profile_Panels1_win_width = 8
                     Profile_Panels1_win_aspect_ratio = 1.25 ! aspect_ratio = height/width

                     Profile_Panels1_xleft = 0.15
                     Profile_Panels1_xright = 0.83
                     Profile_Panels1_ybot = 0.15
                     Profile_Panels1_ytop = 0.9
                     Profile_Panels1_txt_scale = 1.0
                     Profile_Panels1_title = 'Profile Panels1'

                     Profile_Panels1_xaxis_name = 'mass'
                     Profile_Panels1_xaxis_reversed = .false.
                     Profile_Panels1_xmin = 0.22 ! only used if /= -101d0
                     Profile_Panels1_xmax = 0.28 ! only used if /= -101d0
                     Profile_Panels1_xmargin = 0d0
                     Profile_Panels1_show_mix_regions_on_xaxis = .false.

                     Profile_Panels1_yaxis_name(:) = 'Prandtl'
                     Profile_Panels1_yaxis_reversed(:) = .false.
                     Profile_Panels1_yaxis_log(:) = .false. ! show log10 of abs value
                     Profile_Panels1_ymin(2) =  1.337 ! only used if /= -101d0
                     Profile_Panels1_ymax(2) =  1.339 ! only used if /= -101d0
                     Profile_Panels1_ycenter(:) = -101d0 ! only used if /= -101d0
                     Profile_Panels1_ymargin(:) = 0.1
                     Profile_Panels1_dymin(:) = -1

                     Profile_Panels1_other_yaxis_name(:) = ''
                     Profile_Panels1_other_yaxis_reversed(:) = .false.
                     Profile_Panels1_other_yaxis_log(:) = .false. ! show log10 of abs value
                     Profile_Panels1_other_ymin(:) = -101d0 ! only used if /= -101d0
                     Profile_Panels1_other_ymax(:) = -101d0 ! only used if /= -101d0
                     Profile_Panels1_other_ycenter(:) = -101d0 ! only used if /= -101d0
                     Profile_Panels1_other_ymargin(:) = 0.1
                     Profile_Panels1_other_dymin(:) = -1

                     Profile_Panels1_show_grid = .false.

                     ! setup default plot
                     Profile_Panels1_num_panels = 3
                     Profile_Panels1_yaxis_name(1) = 'logT'
                     Profile_Panels1_other_yaxis_name(1) = 'Prandtl'
                     Profile_Panels1_yaxis_name(2) = 'mu'
                     Profile_Panels1_other_yaxis_name(2) = 'he3'!'he3'


                     Profile_Panels1_yaxis_name(3) = 'gradr_sub_grada' !'super_ad'
                     Profile_Panels1_other_yaxis_name(3) = 'gradL_composition_term'!'he3'

                     ! Enables calling a subroutine to add extra information to a plot
                     ! see `$MESA_DIR/star/other/pgstar_decorator.f90`
                     Profile_Panels1_use_decorator = .false.

                     ! file output
                     Profile_Panels1_file_flag = .false.
                     Profile_Panels1_file_dir = 'png'
                     Profile_Panels1_file_prefix = 'profile_panels1_'
                     Profile_Panels1_file_interval = 5 ! output when `mod(model_number,Profile_Panels1_file_interval)==0`
                     Profile_Panels1_file_width = -1 ! (inches) negative means use same value as for window
                     Profile_Panels1_file_aspect_ratio = -1 ! negative means use same value as for window

/ ! end of pgstar namelist



==> table_data_short.tex <==
%\begin{minipage}{1.0\textwidth}
\begin{table}[tb]
\begin{center}
\caption{Observed extra mixing drops in bins of mass and metallicity, corrected for the  0.1456 dex of unmixing observed that we assume is due to systematic errors.} 
\begin{tabular}{rrrr}
\hline
\multicolumn{1}{l}{M} & \multicolumn{1}{l}{[Fe/H]} & \multicolumn{1}{l} {$\Delta$[C/N]$_{\rm APK, cor}$} & {$\Delta$[C/N]$_{\rm Shet, cor}$}   \\ \hline \hline
0.9 & -1.4 & ... & 0.73  \\
0.9 & -1.2 & ... & \multicolumn{1}{r}{0.67}  \\ 
0.9 & -1.0 & ... & \multicolumn{1}{r}{0.48}  \\ 
0.9 & -0.8 & 0.52 & \multicolumn{1}{r}{0.36}  \\ 
0.9 & -0.6 & 0.29 & \multicolumn{1}{r}{0.27}  \\ 
0.9 & -0.4 & 0.16 & \multicolumn{1}{r}{0.21}  \\ 
1.1 & -0.4 & 0.13 & ...  \\ 
1.3 & -0.4 & 0.07 & ...  \\ 
1.5 & -0.4 & 0.10 & ...  \\ 
0.9 & -0.2 & 0.20 & ...  \\ 
1.1 & -0.2 & 0.11 & ... \\ 
1.3 & -0.2 & 0.09 & ...  \\ 
1.5 & -0.2 & 0.10 & ...  \\ 
1.1 & 0.0 & 0.14 & ...  \\ 
1.3 & 0.0 & 0.05 & ...  \\ 
1.5 & 0.0 & 0.09 & ...  \\ 
1.7 & 0.0 & 0.02 & ... \\ 
1.1 & 0.2 & 0.12 & ...  \\ 
1.3 & 0.2 & 0.00 & ... \\ 
1.5 & 0.2 & 0.01 & ...  \\ 
1.7 & 0.2 & 0.00 & ...  \\ 
1.1 & 0.4 & 0.04 & ...  \\ 
1.3 & 0.4 & 0.01 & ...  \\ \hline
\end{tabular}
\label{tab:obsdata}
\end{center}
\end{table}
%\end{minipage}
